A Hierarchical WDM-based Scalable Data Center Network Architecture

Massive data centers are at the heart of the Internet. The rapid growth of Internet traffic and the abundance of rich data-driven applications have raised the need for enormous network bandwidth. Towards meeting this growing traffic demand, optical interconnects have gained significant attention, as they can provide high throughput, low latency, and scalability. In particular, optical Wavelength Division Multiplexing (WDM) provides the possibility to build data centers comprising of millions of servers, while providing hundreds of terabits per second bandwidth. In this paper, we propose a WDM-based Reconfigurable Hierarchical Optical Data Center Architecture (RHODA) that can satisfy future Internet traffic demands. To improve scalability, our DCN architecture is hierarchical, as it groups server racks into clusters. Cluster membership is reconfigurable through the use of optical switches. Each cluster enables heavy-traffic communication among the racks within. To support varying traffic patterns, the inter-cluster network topology and link capacities are also reconfigurable, which is achieved through the use of optical space switches and Wavelength Selective Switches (WSSs). Our simulation results demonstrate that in terms of average hop distance, RHODA outperforms OSA, FatTree and WaveCube by up to 81%, 66% and 60%, respectively.

==> 2_related_work.tex <==
\section{Related Work}\label{sec:relatedwork}
The data center is home to the storage, computation, and applications. Proper planning of the data center network design is critical, and performance, efficiency, and scalability need to be carefully considered. Conventional electrical data center networks are built in a multistage manner to solve the problem. For FatTree \cite{al2008scalable} leverages off-the-shelf Ethernet switches to build large-scale data center networks, and provides high compatibility with existing infrastructure. BCube \cite{guo2009bcube} is a server-centric network structure, and supports various bandwidth-intensive applications. However, throughput and power consumption requirements on massive data centers are the critical challenges for the electrical switches. Our RHODA employs AWGR, which is a passive optical device that can separate and combine signals with different wavelengths, and active optical switches with limited reconfiguration times to solve the problem. AWGR does not require reconfiguration, and can achieve flow contention resolution in the wavelength domain based on its cyclic routing feature.

Some existing optical data center network architectures are AWGR-based. DOS~\cite{ye2010scalable}, Petabit~\cite{xia2010petabit}, PODCA \cite{xu2016podca}, OGDCN~\cite{sankaran2016optical}, F-DCN~\cite{yan2016novel}, POTORI~\cite{cheng2017potori}, Opsquare \cite{yan2017opsquare}, and HiFost~\cite{yan2018hifost} represent the state-of-the-art in terms of AWGR optical switching in high performance data center interconnects. 

The DOS topology consists of an array of tunable wavelength converters (TWC), an AWGR, a loopback shared buffer, and a control panel. The control panel centrally schedules traffic to ensure each node can access any other node through AWGR by configuring the transmitting wavelength of the TWC and the label extractors (LEs). Also, the control panel caches traffic in the shared buffer to avoid contentions among flows. The scalability of the DOS is limited by the scalability of the AWGR and the tuning range of the TWC. As a 512-port AWGR has been presented~\cite{cheung2014ultra}, the DOS architecture can be used to connect up to 512 nodes (assuming that each node is used as a ToR switch or a server switch). The main drawback of the DOS architecture is that it relies on packet buffers for the congestion management using power hungry E/O and O/E converters, thus increasing overall power consumption and the latency. Furthermore, the DOS architecture uses TWCs that are much more expensive than commodity optical transceivers used in current switches, and the scalability of DOS is limited by the size of AWGR and the tuning range of the TWC. 

Petabit~\cite{xia2010petabit} is a three-stage Clos architecture. Each stage consists of an array of AWGRs that are used for routing of packets. The tunable lasers are used for routing the packets through the AWGRs in the first stage. In the second and the third stage, TWCs are used to convert the wavelength and route according to destination of the packet. Different from DOS, Petabit does not rely on any buffers to avoid the power-hungry E/O and O/E conversion. Based on fast tuning rate of TWC (of the order of 100~ns), Petabit can achieve $99.6\%$ throughput even in the case of 10000 ports. In Petabit, between two stages, $M$ TWCs are needed to tune wavelengths, where $M$ is the number of racks. The TWCs bring large cost and power consumption~\cite{chen2015optical}.

PODCA~\cite{xu2016podca} proposes three different-sized architectures. These architectures can achieve low latency and $100\%$ throughput under uniform traffic. For scalability, PODCA adopts a multi-hop routing scheme, instead of single hop as DOS and Petabit. PODCA can accommodate over 2 million servers. However, the main drawback is that PODCA lacks reconfigurability, and it can not configure topology based on features of traffic patterns.

Opsquare \cite{yan2017opsquare} presents a low cost and low power consumption architecture consisting of intra- and inter-cluster networks. However, is not easily scalable with the number of servers. Moreover, inter-cluster switches of Opsquare only connect to a single rack in each cluster, which might result in imbalance of ToR load.

OSA~\cite{ChenOSA} leverages runtime reconfigurable devices, i.e., MEMS and WSS, to dynamically change its topology and link capacity, in order to achieve great flexibility and high performance. OSA can accommodate varying traffic patterns with high bisection bandwidth. The main disadvantage of OSA is that racks with large mutual traffic are not clustered together, and this results in large ToR load and link load. Also, the hop distance between two racks is very large when the number of racks in the network is large.

Different from OSA, WaveCube \cite{chen2015wavecube} does not use MEMS switches. WaveCube achieves scalability, fault-tolerance, and high-performance simultaneously by exploring multi-pathing in the topology. It employs WSSs to provide dynamic link bandwidth adapting to the changing amount of traffic on each output port. However, it is not designed for accommodating different traffic patterns, and the restrictive node count is also a major disadvantage.
